Spectroscopy of SU(4) lattice gauge theory with fermions in the two index anti-symmetric representation

We present a study of spectroscopy of SU(4) lattice gauge theory coupled to two flavors of Dirac fermions in the anti-symmetric two index representation. The fermion representation is real, and the pattern of chiral symmetry breaking is SU(2Nf) -> SO(2Nf) with Nf flavors of Dirac fermions. It is an interesting generalization of QCD, for several reasons: it allows direct exploration of an alternate large Nc expansion, it can be simulated at non-zero chemical potential with no sign problem, and several UV completions of composite Higgs systems are built on it. We present preliminary results on the baryon and meson spectra of the theory and compare them with SU(3) results and with expectations for large Nc scaling.

==> Makefile <==

TEXFILES= main.tex

paper: Makefile $(BIBFILES) $(TEXFILES)
	latex main.tex && \
	latex main.tex && \
	dvips main.dvi && \
	ps2pdf -dNOSAFER main.ps

view: 
	#acroread main.pdf
	evince main.pdf

clean:
	rm -f *.log *.aux *.out *~ *.dvi

distclean: clean
	rm -f *.bbl *.blg main.ps main.pdf *~ *.dvi

